Reconstruction as Spatial Evaluation: Diagnosing Cross-View Spatial Intelligence in Large Vision-Language Models

The spatial intelligence of large vision-language models (LVLMs) requires the ability to combine local visual observations into a geometrically consistent representation of the physical world. Many static benchmarks assess isolated spatial judgments, such as relative direction or distance, while interactive embodied evaluations combine perception with exploration, planning, control, and simulator-specific execution. To bridge this gap, we introduce RECONSPATIAL, a benchmark centered on multi-view 3D scene reconstruction across indoor, tabletop, and outdoor environments. Given real multi-view images and target-object queries, LVLMs are required to jointly predict oriented 3D bounding boxes in a shared, camera-anchored metric coordinate frame. Reconstructions are evaluated along two complementary axes: Structure for relative layout and Metric for physical scale and camera-anchored placement. Nine atomic spatial QA tasks, grouped into Geometric Perception and Spatial Relations, probe spatial capabilities involved in joint reconstruction. Offline navigation extends evaluation to path planning. Evaluation of 18 frontier LVLMs reveals a consistent gap between relative scene structure and metric reconstruction; even GPT-6-Astra scores 81.4% on Structure but only 58.7% on Metric. Tracing this gap, diagnostic analyses link atomic spatial capabilities to reconstruction quality and show that relational consistency alone does not ensure metric accuracy. Experiments with 3D map injection further separate scene construction from path planning, revealing how these geometric errors limit navigation success. Finally, spatial fine-tuning yields broad transfer across both spatial and general vision-language benchmarks.

==> layout_helpers.tex <==
\newsavebox{\rightinsetbox}
\newsavebox{\rightinsetparagraph}
\newcount\rightinsetlines
\makeatletter
\newenvironment{rightinsettext}[3]{%
  \par\begingroup
  \sbox{\rightinsetbox}{%
    \begin{minipage}[t]{#2}%
      \vspace{0pt}%
      \def\@captype{#1}%
      #3%
    \end{minipage}}%
  \begin{lrbox}{\rightinsetparagraph}%
  \begin{minipage}[t]{\linewidth}%
    \vspace{0pt}%
    \rightinsetlines=\dimexpr\ht\rightinsetbox+\dp\rightinsetbox+1.5\baselineskip\relax
    \divide\rightinsetlines by \number\baselineskip
    \hangafter=-\rightinsetlines
    \hangindent=-\dimexpr\wd\rightinsetbox+1em\relax
    \noindent\ignorespaces
}{%
    \par
  \end{minipage}\end{lrbox}%
  \noindent\rlap{%
    \hspace*{\dimexpr\linewidth-\wd\rightinsetbox\relax}%
    \usebox{\rightinsetbox}}%
  \usebox{\rightinsetparagraph}\par
  \endgroup
}
\makeatother

